MarioMix: Creating Aligned Playstyles for Bots with Interactive Reinforcement Learning

In this paper, we propose a generic framework that enables game developers without knowledge of machine learning to create bot behaviors with playstyles that align with their preferences. Our framework is based on interactive reinforcement learning (RL), and we used it to create a behavior authoring tool called MarioMix. This tool enables non-experts to create bots with varied playstyles for the game titled Super Mario Bros. The main interaction procedure of MarioMix consists of presenting short clips of gameplay displaying precomputed bots with different playstyles to end-users. Then, end-users can select the bot with the playstyle that behaves as intended. We evaluated MarioMix by incorporating input from game designers working in the industry.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


==> marioMix_scribendi.tex <==
abstract
In this paper, we propose a generic framework that enables game developers, without knowledge in machine learning, to create bot behaviors with playstyles that align with their preferences. Our framework is based on interactive reinforcement learning (RL) and we used it to create the behavior authoring tool called MarioMix. This tool enables non-experts to create bots with varied playstyle for the game named Super Mario Bros. The main interaction procedure of MarioMix consist on presenting to the end-users short clips of gameplay displaying pre-computed bots with different playstyles. Then, the end-users can select the bot with the playstyle that behaves as they intended. We evaluated MarioMix with game designers working in the industry.

\section{Introduction}
\label{sec::Introduction}
Research on artificial intelligence (AI) for games is going through an era of rapid advances in many different areas. However, these novel approaches are rarely adopted by the game industry; academic research on AI for games (game AI) and AI development in commercial games are focused on different problems \cite{Yannakakis2015Panorama}. While academic researches aim to create automatic AI techniques for general proposes, game designers prefer robust techniques that perform as they intend in a particular application. 

For instance, creating bots with varied playstyles can be useful for game designers in early development stages, such as playtesting using bots \cite{Ariyurek2019, Pfau2018}. Unfortunately, such bot behaviors have not been widely adopted in the game industry. This is because creating bots with varied playstyles is time-consuming and often requires end-users with knowledge in machine learning \cite{Hohman2018, Yang2019, Greydanus2018}. On top of that, designing a playstyle that aligns with the game designer intentions is a major challenge in the AI research field \cite{Leike2018}. In this paper, we propose a generic framework based on interactive reinforcement learning (RL) \cite{Fails2003, Amershi2014, Sacha2016} that will enable the design of authoring tools for bot behaviors with playstyles that align with the intention of end-users without knowledge on RL.

The interactive RL setting involves a human-in-the-loop that gives feedback to the underlying RL algorithm to improve its performance or guide it to solve a problem in a particular manner \cite{Amershi2014, Leike2018}. One major challenge in interactive RL is making it usable in high-dimension environments since most interactive RL-based applications require up to millions of human feedback samples to get good results \cite{Arzate2020, Griffith2013, Li2013, Rosenfeld2018}. To overcome the sample inefficiency of current interactive RL methods, our framework proposes a novel interaction procedure that consists on mixing pre-computed policies, and a search method for finding the playstyle that fits the end-users' preferences.  

The mixture of policies is performed by assigning different policies (each policy exhibits a different playstyle) to specific segments of a game level. A similar interaction is proposed in \cite{Sorensen2016}, where users can guide an interactive evolutionary computation (IEC) \cite{Takagi2001} based algorithm by deciding which individuals (or behavior) are used for breeding in the next iteration of the evolutionary algorithm. The main differentiation between the IEC-based algorithm in \cite{Sorensen2016} and our work is that we can achieve short interaction cycles because we follow a top-down method that only requires the users to evaluate short gameplay clips, and selecting which one is their favorite. Furthermore, the computation of the behaviors is done offline -- end-users do not need to wait for any computation while they use a tool based on our generic framework.

As a proof-of-concept of this framework, we build a tool designed around it called MarioMix. The aim of MarioMix is to create aligned playstyles for bots in a clone of the \textit{Super Mario Bros.} video game. Finally, we avaluate MarioMix with a user study in which professional game developers working in the industry participated. The results of our study reveal that MarioMix is an effective tool for creating aligned bot behaviors through interactive RL for a game industry context.


\section{Related Work}
\label{sec::RelatedWork}
Most research on ML focuses on algorithms that automatically finds a solution for a particular problem. On the other hand, we find iML \cite{Fails2003} incorporates a human-in-the-loop that integrates their domain knowledge to enhance the solution of the model at hand. In this paper, we focus on interactive RL based approaches for agent alignment (we refer our readers interested in agent alignment to the survey on this subject in \cite{Leike2018}). That is, our research scope includes works that use interactive RL to generate agent behaviors that characterize the end-users intentions.

\subsection{Interactive Reinforcement Learning}
There is extensive research on interactive Reinforcement Learning (RL) \cite{Arakawa2018, Rosenfeld2018, Elizalde2012, Korpan2017, Wang2018, McGregor2017, Griffith2013, Li2013, Amir2016, Fachantidis2017}. For a survey on interactive RL, please refer to \cite{Arzate2020}. 

Arguably, one of the most common approach in interactive RL is policy shaping (PS) \cite{Griffith2013}. The basic idea of PS is to augment the policy of an RL model using human feedback. This feedback can be an action advice \cite{Macglashan2017, Krening2018}, or a critique \cite{Griffith2013, Krening2018}. In action advice, users provides to the model feedback on what they think is the optimal action to perform in a particular state. While a critique consists of binary feedback that indicates if a performed action by the bot, at a given state, is good or not. 

In contrast, our framework uses a PS method but at a higher-level since we mix policies and each of them activates at a predefined space in the game level. This PS approach has the advantage of fast interaction cycles, which is essential to avoid the fatigue of users. Furthermore, by using precomputed policies, we enable the use of interactive RL in a complex environment such as \textit{Super Mario Bros}.

There are other alternatives to provide action advice or feedback to an agent such as using apprentice learning \cite{Abbeel2004}, inverse RL \cite{Ng1999, Ziebart2008, Ziebart2009}, or from demonstration \cite{Taylor2011}. All these techniques use as input demonstrations of a user of how a bot is supposed to perform a certain task. 
 
Our framework also uses human feedback in the form of gameplay demonstrations in a similar manner to the works in \cite{Taylor2011, Ng1999, Ziebart2008, Ziebart2009, Abbeel2004}. However, unlike those approaches, our framework uses the gameplay demonstrations for searching in the playstyle space. That is, we characterize the playstyle of the users, and then we present to them the bot with the most similar playstyle to theirs in our behavior dataset. This interaction channel is aimed at reducing the needed time and feedback for alignment problem \cite{Griffith2013, Li2013, Rosenfeld2018}.

\subsection{AI-assisted tools for agent behavior}
AI tools have been used extensively for Procedural Content Generation (PCG) \cite{Summerville2018, Roberts2015, Khalifa2016, Sheffield2018}. However, the application of AI-assisted tools for agent behavior is still underexploited; must approaches focus on automatic generation of agent behavior (for a survey on this subject, refer to \cite{Yannakakis2015Panorama}). 

For instance, the NERO platform has the objective of generating believable behaviors for a first-person shooter \cite{Stanley2005}. This neuroevolution-based approach has the particularity of improving the performance of its agents by allowing imitation learning the agent learns from demonstration a policy that mimics the expert's trajectory \cite{Abbeel2004, Finn2016, Ho2016}. Another example can be found in \cite{Sorensen2016} where an interactive evolutionary computation (IEC) approach \cite{Takagi2001} is implemented. In this application, users have the task of guiding an evolutionary algorithm by selecting which bots will be used for breeding in the next iteration or die. 

In our generic framework, we use interactive RL instead of IEC like in the previously mentioned works. In a similar manner to the NERO platform \cite{Stanley2005}, we use gameplay trajectories as input, however, we use them as a search method in the playstyle space. The interaction procedure in MarioMix is similar to the work in \cite{Sorensen2016}, since we also present to the user clips of different playstyle behaviors. However, we use this interaction procedure to generate a mixture of policies with varied playstyles that align with the user preferences.
 

\section{Proposed Approach}
\label{sec::Approach}
The components of our generic framework are: a problem expressed as a Markov Decision Process (MDP) (either flat or hierarchical), an algorithm that solves the MDP(s), a dataset of policies (each of them with a distictive playstyle), a search function for the playstyle space, a playstyle similarity metric, and a method for delimiting the activation of the policies.

\subsection{MDP solver}
For creating the policy dataset we use the model-based reinforcement learning (RL) architecture called HRLB\textasciicircum2 \cite{Arzate2018}. We chose this architecture because it let us do reward shaping while avodinf re-training the bot evrytime we design a new reward function. Also, it allow us to assign a reward to both states in the environment or actions of the bot. 

\subsection{Policy dataset}
We create distictive playtyles for the policy dataset through reward shaping (RS). That is, we manually design a particular reward function so the resulting policy has a unique playtyle. Finally, we store all policies in our policy dataset, and for each of them, we also compute its playstyle similarity metrics. 

\subsection{Playstyle similarity metric}
\label{subsec::similaritymetric}
The playstyle similarity metric is dsigned to characterize, in a quantitative manner, the playstyle of each policy. To do that, we keep track of the frequency of use of each action, and the visiting frequency of each state in the environment. 

\subsection{Search function}
Our framework provides a function that allows user to search for policies in pur dataset that exhibit the desired playstyle. This search function can either use as input gameplay traces fro the users, or a policy in our dataset. For the first option, users take control of the character in the game and demonstrate the playstyle they are looking for. Once the users end the gameplay demonstration, our framework characterize their playtyle and provides as output the policy in our dataset that better resemble their exhibited gameplay plan. The second option dor searching takes as input one of the policies in our dataset; users only need to select the preferred policy/plasytyle as input, and our framework will provide the closest playstyle to this input in our dataset. 

To compute the similarity between playstyles, we use the mean squared error to estimate the difference between the playstyle metrics. 


\subsection{Delimiting the activation of the policies}
The end-user should be able to delimit the activation of each policy that shapes the entire playstyle of the bot, depending on the game, this procedure might vary. For instance, in a platforming game we could delimit the activation of a policy to a determined segment in a game level. On the other hand, for a fighting game we could assign an specific policy according to the health level of the bot. 

\section{MarioMix}
\label{sec::MarioMix}
Based on the generic framework we proposed in the last section, we designed the authoring tool called MarioMix. This tool is aimed at creating aligned behaviors for the game \textit{Super Mario Bros.}, where the end-users  

Interface
In Figure \ref{Fig:mainInterface}, we display the MarioMix interface, let us introduce its elements trough an example of the user study we explain in Section \ref{sec::UserStudy}. 

In this example, a game developer named Sophia wants to create a synthetic tester for Super Mario Bros. using MarioMix. First, she selects the desired game level and the resolution of the segments using the corresponding controls in panel \textbf{(b)}. Sophia can select the game level to display using the drop-down list and ``Load'' button on the top right corner of the panel. Furthermore, she can change the resolution of the current game level with the slider on the top left corner of the panel. This slider has three different positions, and it controls the number of segments in which a game level is segmented. We segment the game levels in $3$, $5$, and $10$ parts for the low, medium, and high resolutions, respectively. 

Now Sophia can focus on assigning playstyles to all the segments in the game level that are presented in panel \textbf{(a)}. From this panel, she can select a segment to work with by clicking on the corresponding checkbox on top of each segment thumbnail. Below each thumbnail, the name of the assigned playstyle is presented. Also, this element provides to Sophia with an overview of their current progress on designing a mixture of playstyles for the whole game level at hand.

The next step is finding the right playstyle for each segment. To do that, Sophia starts by reviewing the two proposed playtyles by MarioMix (in the first iteration, MarioMix presents two playtyles at random) using the buttons in panel \textbf{(d)}. By pressing the button ``Play fullscreen'' on the left of the panel, only the playstyle option on the left is displayed using all the space in \textbf{(c)}; the function of the ``Play fullscreen'' on the right is similar but for the playstyle option on the right. On the example in Figure \ref{Fig:mainInterface}, the left, and right behavior options are Playstyle $5$ and Playstyle $9$, respectively. The button on the center, ``Play Both'', displays both playstyle options at the same time.

However, Sophia did not find the type of playstyle she wants in either Playstyle $5$ nor $9$. So she decides to explore the playstyle space using her own gameplay as input. She starts this process by pressing the ``From demonstration'' button in panel \textbf{(b)}. After pressing this button, a window with the game is shown in the \textit{game display zone} \textbf{(f)} with the game character in the start position of the current game level. In this game window, Sophia has control of the main character, Mario. Once the character dies, or Sophia decides to close the game window, her playstyle metrics are computed. Then, by pressing the ``Display Options'' button in panel \textbf{(b)}, MarioMix presents to Sophia (on the \textit{game display zone}) the two most similar playstyles that match her exhibited behavior.

This time, the Sophia likes one of the proposed playstyles by MarioMix, however, she thinks it is a bit off to what she wants, so she keeps exploring the plastyle space now using this suggested playtyle behavior as input. To do that, she first selects the input behavior using the checkboxes in panel \textbf{(e)}, and then she presses the ``More'' button in the same panel. By doing that, MarioMix searches a different behavior that is similar to the one selected in the checkboxes and display it in the \textit{game display zone}. This time, Sohpia finds the perfect playtyle so she selects in the checkboxes and then press the button ``Assign''.

After assiging the perfect playtyles for the segments that Sophia considers the most important, she is ready to see how Mario plays the whole game level. Therefore, she uses the automatically assign so MarioMix finishes her job. By pressing the ``Automatically Assign'' button, MarioMix automatically assigns a behavior to the segments without an assigned behavior (or marked as ``No Behavior Selected''). The heuristic to select a behavior is to start from the first segment and repeat the selection of behavior by Sophia to those unassigned segments. If any segment has a playstyle assigned, MarioMix takes on playstyle at random from the dataset and assign it to the whole game level at hand.

Once Sophia finishes assigning plasytyles to all the segments in the game level, she decides to review how Mario plays. The tools for reviewing the assigned playstyles are two buttons and the drop-down menu on the bottom right corner of panel \textbf{(b)}. When Sophia presses the ``Review Level'' button, MarioMix displays the bot playing with the designated playstyles on the \textit{game display zone}. Besides, the panel \textbf{(f)} informs her about the current segment, and playstyle, that the bot is playing. However, if Sophia prefers to review only a particular segment, she can do that with the button ``Review Segment'' and the drop-down menu next to it; if she clicks on this button, MarioMix displays the bot playing the selected segment in the drop-down menu.



\section{Bot Definition}
\label{sec::BotDefinition}
In this section, we explain how we discretized the game Super Mario Bros. for MarioMix. Additionaly, we present the handcrafted reward functions that we used to regenrate varied playtyles.

\subsection{State representation}
For the representation of Super Mario Bros. as a Markov Decision Process (MDP), we use a $3 \times 3$ grid of variables that code terrain information. This grid can recognize between platforms, coin blocks, and coins. Also, our MDP takes into account the position (in $X$ and $Y$ axes) of the two nearest enemies to Mario. The position variables are discretized into $7$ values that go from $0$ to $6$. We also added a binary variable that detects if there's a cliff in front of Mario or not.

Our bot can perform $10$ different actions. Mario performs the next actions for both the left and right side of the screen: actions walk, run, jump, and quick jump. Furthermore, Mario can do nothing, and neutral jump.

\subsection{Policy dataset}
\label{subsec::RewardFunctions}
In order to create multiple playstyles for our policy dataset, we hand-engineered $11$ reward functions (RFs). These RFs are aimed to generate a wide range of playstyles, within the range that our discretization allows us.

First, we focus on creating policies that maximized the next behavior traits in the bot: the speed at completing the level, how it overcomes enemies, how it approaches coins, and how often it jumps. For the speed trait, we designed RFs that created bots that either was very quickly at advancing in the level, or slow. Regarding how the bot overcomes enemies, we crafted RFs that made the bot very cautious about enemies (it avoided them as much as possible), or highly possible to kill them. Also, we have RFs that create bots that collect as many coins as possible, or that they don't care about them. Finally, for the jump preference, some bots jump as much as possible, while others avoid jumping. 

With the aforementioned base playstyle as a basis, we combined them to create $11$ unique bot behaviors for MarioMix.


\section{User Study}
\label{sec::UserStudy}
For the user study of MarioMix, two expert game developers (employed in the game industry and without knowledge on academic machine learning) were asked to create bot behaviors for three game levels of Super Mario Bros. Given the current situation regarding COVID-19, these expert users tested MarioMix remotely. After the completion of the task given to the experts, we asked them a few questions about the usability of MarioMix through an online survey. Additionally, we asked for more feedback via phone and e-mails.

\subsection{Task}
We presented MarioMix to the experts as a tool to design varied behaviors for synthetic testers; or bots that are intended to playtest a game automatically. Therefore, experts focused on crafting a mixture of behaviors that are intended to playtest Super Mario Bros. They put special attention on how the bot plays in specific situations. For example, how the bot handles to survive a specific group of enemies in the level.

The complete task for the expert users is to create a mixture of behaviors for three different game levels in MarioMix.


\subsection{Survey}
Once the experts completed the assigned task, they took a survey with the next closed-ended questions:

\begin{enumerate}
  \item Have you ever played the game called Super Mario Bros.? with options: Yes, No, I've only watched other people playing it
  
  \item Would you like to have a tool like MarioMix for your current game you are developing? with options: yes, no

  \item How close are the bot behaviors you created to what you had envisioned? with options not similar at all, some resemblance, very similar, perfect match
\end{enumerate}

Then, we asked the expert users open-ended questions to better understand their most effective workflow while using MarioMix:

\begin{enumerate}
  \item How would you describe the most effective workflow using MarioMix?
  
  \item Which was your preferred resolution and why?

  \item Which way of watching behavior options do you prefer? (two at the same time or one by one) 
\end{enumerate}

Finally, we talked with the experts to get more general comments about the usability of MarioMix in an industry context.



\section{Results}
\label{sec::Results}
Overall, participants of our user study responded positively to the MarioMix interaction method for creating bot behavior. Both experts agree that the interaction procedure of MarioMix is effective at creating bot behaviors that align with their intentions. Moreover, the participants found entertaining the evaluation procedure; they found interesting, and effective, to evaluate bot playstyle by observing short gameplay clips.

The participants spent between $40$ and $60$ minutes using MarioMix. First, we gave them a short demonstration of the capabilities of MarioMix and explained to them the task they have to perform. After they completed the task, we conducted the survey.

Regarding the closed-ended questions in our survey, \textbf{(1)} all participants have played before Super Mario Bros., and \textbf{(2)} they would like to have a tool like MarioMix for creating bot behaviors for their games. On \textbf{(3)} how close the final behaviors were to what they had envision, the answers were: some resemblance, and very similar. 

The responses for the open-ended question \textbf{(1)} revealed that both participants had a similar method for using MarioMix. As a first step, participants tried the different resolutions, after a couple of minutes testing, they chose one and kept it for the rest of the task. From here, they prefer to try first the behaviors suggested by default in different segments; when they found they did not like any of the playstyles at hand for a particular segment, they explored the dataset using the ``More'' function. This exploration procedure continued for a few iterations, if they did not find a compelling playstyle, then they change their search procedure to use the ``From Demonstration'' approach. Once they assigned all segments a playstyle, they reviewed the whole game level using the ``Review Level'' function. If they found a problem in a segment, they went back to find a new playstyle that better fitted that part of the game level.

For question \textbf{(2)} in the open-ended section, both participants preferred to use a medium resolution ($5$ segments per game level). Experts mentioned that the high-resolution segments were too short for a correct assessment of the playstyles, while the low resolution does not provide enough control to make the bot play as they intended in certain areas of the game level. From low to high, the mean durations of gameplay clips are $2.5$, $5.2$, and $8.7$ seconds.

The answers for the open-ended question \textbf{(3)} reveal that playing both behavior options side by side is the more effective for a quick preference evaluation. Participants reported that by watching both playstyles at the same time they can get a broad understanding of the behaviors and how they compare to each other; which makes it easy to spot unwanted traits. However, when participants are looking for a particular feature in the behavior, it was better to examine one playstyle at a time. The usual procedure was to do a coarse assessment by watching both playstyles at the same time and then refine the search by watching one playstyle at a time.

In regards to the interface, experts would like to have more control over the creation of segments. In particular, they mentioned that they would like to be able to manually create the segments so they can give more resolution to the parts of the game level they consider more relevant.

It's worth mentioning that participants also found the ``More'' option compelling because it let them find playstyles that they haven't thought they were appropriate for performing tests. That is, this kind of exploration provides users a wider view of possible ways to play the game at hand.

Moreover, the experts pointed out that the ``From Demonstration'' approach is useful in most cases since it helped them to find the required playstyle. However, it did not perform well when participants were looking for a precise gameplay trace. For instance, ``I'd like that Mario kills the Koopa Troopa and then hit the shell to kill the rest of enemies ''. Since our playstyle similarity metric characterizes the behavior of the character in a more general manner, we cannot these kinds of specific events in gameplay.

\section{Discussion and Future Work}
\label{sec::Discussion}
From the user study, we can conclude that the top-down method of our generic framework for tackling the agent alignment problem is effective; the participants consider that the behaviors they created for synthetic testers are close enough to their intentions to be useful in a real-world scenario. Nevertheless, they would like to be able to create more precise behaviors for certain events in the game. Also, the small number of policies in our dataset limits the variety of plasytyles that users can generate. These obervations propose new challenges: how to automatically create a more diverse number of policies/playstyles, and how to create such accurate bot behaviors while minimizing the needed feedback from users. 

The positive outcomes of the user study validate MarioMix as an effective tool that game developers, without knowledge on academic machine learning (ML), can create effective bot behaviors. However, adapting MarioMix for different games would require an expert on ML to do it. As future work, we would like to investigate on how to create tools for non-experts in ML to enable them to adapt tools like MarioMix to be used in other games. As far as we know, this research direction is unexplored.

Although the fact that professional game developer were involved in the user study increases the ecological validity of our results, we still need to perform more tests to confirm the generalization of our claims. To fully validate our generic framework, we would like to adapt more games of different genres to use it and test them with more professionals in the game industry. However, the results of the presented preliminary evaluation are promising.

Finally, one advantage of model-based reinforcement learning is that we can easily change the reward function of a bot to adapt its behavior. We would like to explore the creation of companions \cite{Emmerich2018} that adapt according to the preferences of the game developers. 


\section{Conclusions}
\label{sec::Conclusions}
In this paper, we presented a generic framework for creating aligned bot behaviors. In particular, our proposed approach provides users with novel interaction procedures that allow them to create personalized bot behaviors with a top-down method; which consist on evaluating short gameplay clips.

As a proof-of-concept of our framework, we build a tool designed around it called MarioMix. This tool was evaluated by game developers working in the game industry. The preliminary results of this evaluation are positive: experts agree that their current workflow would be benefited by a tool like MarioMix. Furthermore, these results are encouraging for the adoption of academic AI techniques in commercial games. 

